VNT-Net: Rotational Invariant Vector Neuron Transformers

Learning 3D point sets with rotational invariance is an important and challenging problem in machine learning. Through rotational invariant architectures, 3D point cloud neural networks are relieved from requiring a canonical global pose and from exhaustive data augmentation with all possible rotations. In this work, we introduce a rotational invariant neural network by combining recently introduced vector neurons with self-attention layers to build a point cloud vector neuron transformer network (VNT-Net). Vector neurons are known for their simplicity and versatility in representing SO(3) actions and are thereby incorporated in common neural operations. Similarly, Transformer architectures have gained popularity and recently were shown successful for images by applying directly on sequences of image patches and achieving superior performance and convergence. In order to benefit from both worlds, we combine the two structures by mainly showing how to adapt the multi-headed attention layers to comply with vector neurons operations. Through this adaptation attention layers become SO(3) and the overall network becomes rotational invariant. Experiments demonstrate that our network efficiently handles 3D point cloud objects in arbitrary poses. We also show that our network achieves higher accuracy when compared to related state-of-the-art methods and requires less training due to a smaller number of hyperparameters in common classification and segmentation tasks.

==> checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}



\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We will publish the code after the paper is accepted}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}



\end{enumerate} 

==> figures/VNT.tex <==
\begin{figure}
\centering
\includegraphics[height=.50\linewidth]{image/VNT.pdf}
\caption{The classification network}. 
\label{fig:VNT}
\end{figure}

==> figures/attentionmap.tex <==
\begin{figure*} [ht]
    \centering
    \includegraphics[width=0.5\linewidth]{image/firstfig.png}
   \caption{\textbf{VNAttention} attention matrix rows map on their input}
   \label{fig:phyDnet_arch}
\end{figure*}

==> figures/dotprod.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.25\linewidth]{image/dotprod.pdf}
    \caption{Vector Scaled Dot-Product Attention using the flatting optimization \ref{optimization}}
\end{figure}

==> overview.tex <==
\section{Overview}




==> tables/class_and_seg.tex <==
\begin{table}[h!]
\centering
\resizebox{.5\textwidth}{!}{%
\begin{tabular}{c c c c}
\hline
Methods               & z/z           & z/SO(3)       & SO(3)/SO(3)   \\ \hline
PointNet \cite{qi2017pointnet}           & 85.9          & 19.6          & 74.7          \\
DGCNN \cite{wang2019dynamic}             & 90.3          & 33.8          & 88.6          \\
VN-PointNet \cite{deng2021vn}            & 77.5          & 77.5          & 77.2          \\
VN-DGCNN    \cite{deng2021vn}            & 89.5          & 89.5          & 90.2          \\ \hline
PCNN \cite{atzmon2018point}              & 92.3          & 11.9          & 85.1          \\
ShellNet \cite{zhang2019shellnet}        & \textbf{93.1} & 19.9          & 87.8          \\
PointNet++ \cite{qi2017pointnetpp}       & 91.8          & 28.4          & 85.0          \\
PointCNN \cite{li2018pointcnn}           & 92.5          & 41.2          & 84.5          \\
Spherical-CNN \cite{esteves2018learning} & 88.9          & 76.7          & 86.9          \\
$a^3$S-CNN \cite{liu2018deep}            & 89.6          & 87.9          & 88.7          \\ \hline
SFCNN \cite{rao2019spherical}            & 91.4          & 84.8          & 90.1          \\
TFN \cite{thomas2018tensor}              & 88.5          & 85.3          & 87.6          \\
RI-Conv \cite{zhang2019rotation}         & 86.5          & 86.4          & 86.4          \\
SPHNet \cite{poulenard2019effective}     & 87.7          & 86.6          & 87.6          \\
ClusterNet \cite{chen2019clusternet}     & 87.1          & 87.1          & 87.1          \\
GC-Conv \cite{zhang2020global}           & 89.0          & 89.1          & 89.2          \\
RI-Framework \cite{li2021rotation}       & 89.4          & 89.4          & 89.3          \\ \hline
\textbf{VNT}                                              & 89.2          & 89.2          & 88.6          \\
\textbf{VNT +N}                                           & 90.3          & \textbf{90.3} & \textbf{90.3} \\
Point Transformer \cite{2021hengshuang}  & 89.0          & 31.0          & 86.1          \\
PCT \cite{2021PCT}                       & 90.0          & 28.3          & 87.0          \\ \hline
SFCNN \cite{rao2019spherical}            & 92.3          & 85.3          & 91.0          \\
LGR-Net \cite{zhao2019rotation}          & 90.9          & 90.9          & 91.1          \\ \hline
\end{tabular}%
}
\caption{Test classification accuracy on the ModelNet40 dataset \cite{wu20153d}in three train/test scenarios. $z$ stands for aligned data augmented by random rotations around the vertical axis and $\mathrm{SO}(3)$ indicates data augmented by random rotations.}
\label{tab:exp:cls}
\end{table}



\begin{table}[h!]
    \centering
    \resizebox{.5\textwidth}{!}{%
    \begin{tabular}{ccc}
    \hline
    Methods                                                 & z/SO(3)       & SO(3)/SO(3)   \\ \hline
    PointNet \cite{qi2017pointnet}        & 38.0          & 62.3          \\
    DGCNN \cite{wang2019dynamic}          & 49.3          & 78.6          \\
    VN-PointNet \cite{deng2021vn}         & 72.4          & 72.8          \\
    VN-DGCNN \cite{deng2021vn}    & \textbf{81.4} & \textbf{81.4} \\ \hline
    PointCNN \cite{li2018pointcnn}         & 34.7          & 71.4          \\
    PointNet++ \cite{qi2017pointnetpp}     & 48.3          & 76.7          \\
    ShellNet \cite{zhang2019shellnet}      & 47.2          & 77.1          \\ \hline
    RI-Conv \cite{zhang2019rotation}       & 75.3          & 75.3          \\
    TFN \cite{thomas2018tensor}            & 76.8          & 76.2          \\
    GC-Conv \cite{zhang2020global}         & 77.2          & 77.3          \\
    RI-Framework \cite{li2021rotation}     & 79.2          & 79.4          \\
    LGR-Net\cite{zhao2019rotation}         & 80.0          & 80.1          \\ \hline
    \textbf{VNT+N}                                          & 80.5          & 80.5          \\
    Point Transformer\cite{2021hengshuang} & 70.3          & 40.8          \\
    PCT\cite{2021PCT}                      & 77.4          & 43.5
    \end{tabular}%
    }
    \caption{ShapeNet part segmentation. The results are reported in the overall average category to mean IoU over 16 categories in two train/test scenarios. With $z$, we refer to data augmented only by random rotations around the vertical axis, and $\mathrm{SO}(3)$ indicates random rotations.}
    \label{tab:exp:seg}
    \end{table}


    
